Energizing Star Formation: The Cosmic Ray Ionization Rate in NGC 253 Derived From ALCHEMI Measurements of H$_3$O$^+$ and SO

The cosmic ray ionization rate (CRIR) is a key parameter in understanding the physical and chemical processes in the interstellar medium. Cosmic rays are a significant source of energy in star formation regions, which impacts the physical and chemical processes which drive the formation of stars. Previous studies of the circum-molecular zone (CMZ) of the starburst galaxy NGC 253 have found evidence for a high CRIR value; $10^3-10^6$ times the average cosmic ray ionization rate within the Milky Way. This is a broad constraint and one goal of this study is to determine this value with much higher precision. We exploit ALMA observations towards the central molecular zone of NGC 253 to measure the CRIR. We first demonstrate that the abundance ratio of H$_3$O$^+$ and SO is strongly sensitive to the CRIR. We then combine chemical and radiative transfer models with nested sampling to infer the gas properties and CRIR of several star-forming regions in NGC 253 due to emission from their transitions. We find that each of the four regions modelled has a CRIR in the range $(1-80)\times10^{-14}$ s$^{-1}$ and that this result adequately fits the abundances of other species that are believed to be sensitive to cosmic rays including C$_2$H, HCO$^+$, HOC$^+$, and CO. From shock and PDR/XDR models, we further find that neither UV/X-ray driven nor shock dominated chemistry are a viable single alternative as none of these processes can adequately fit the abundances of all of these species.

==> emaillist.tex <==
\email{holdship@strw.leidenuniv.nl, eb7he@virginia.edu, viti@strw.leidenuniv.nl, hunt@arcetri.astro.it, jmangum@nrao.edu, harada@asiaa.sinica.edu.tw, Sergio.Martin@eso.org, nakanisi.k@nao.ac.jp, mullers@chalmers.se, rherrero@eso.org, adamginsburg@ufl.edu, chenkel@mpifr-bonn.mpg.de, saalto@chalmers.se, pvdwerf@strw.leidenuniv.nl, aladro@mpifr-bonn.mpg.de, david.meier@nmt.edu, phumire@mpifr-bonn.mpg.de, vmrivilla@gmail.com, lcolzi.astro@gmail.com, s.gburillo@oan.es, kkohno@ioa.s.u-tokyo.ac.jp, t.greve@ucl.ac.uk, g.fuller@manchester.ac.uk, yongxiong.wang@postgrad.manchester.ac.uk, yuri@ioa.s.u-tokyo.ac.jp, takuma.izumi@nao.ac.jp,  takano.shuro@nihon-u.ac.jp, muehle@astro.uni-bonn.de, mamiko@chalmers.se, ktanaka@phys.keio.ac.jp, ksakamoto@asiaa.sinica.edu.tw, yyoshimura@ioa.s.u-tokyo.ac.jp, nakajima@isee.nagoya-u.ac.jp}


==> figures/final_results.tex <==
\begin{tabular}{lrlrlrl}
\toprule
Region &  $n_{H2}$ / \SI{e6}{\per\centi\metre\cubed} & $n_{H2}$ Range &  N$_{H2}$ / \SI{e23}{\per\centi\metre\squared}  & N$_{H2}$ Range &  $\zeta$ / \num{e4} $\zeta_0$  & $\zeta$ range \\
\midrule
     4 &                                         1.4 &      0.7 - 3.3 &                                             5.6 &     2.2 - 12.9 &                            8.2 &    2.2 - 30.8 \\
     5 &                                         1.2 &      0.6 - 2.5 &                                             3.7 &      1.8 - 8.1 &                            7.1 &    2.2 - 26.3 \\
     6 &                                         1.5 &      0.8 - 3.6 &                                             6.7 &     2.1 - 15.7 &                            6.3 &    1.9 - 22.3 \\
     7 &                                         0.1 &      0.0 - 0.5 &                                             3.8 &     1.6 - 12.4 &                            0.9 &     0.2 - 6.8 \\
\bottomrule
\end{tabular}

